Automatic Parallelization of Python Programs for Distributed Heterogeneous Computing

This paper introduces a novel approach to automatic ahead-of-time (AOT) parallelization and optimization of sequential Python programs for execution on distributed heterogeneous platforms. Our approach enables AOT source-to-source transformation of Python programs, driven by the inclusion of type hints for function parameters and return values. These hints can be supplied by the programmer or obtained by dynamic profiler tools; multi-version code generation guarantees the correctness of our AOT transformation in all cases. Our compilation framework performs automatic parallelization and sophisticated high-level code optimizations for the target distributed heterogeneous hardware platform. It includes extensions to the polyhedral framework that unify user-written loops and implicit loops present in matrix/tensor operators, as well as automated section of CPU vs. GPU code variants. Further, our polyhedral optimizations enable both intra-node and inter-node parallelism. Finally, the optimized output code is deployed using the Ray runtime for scheduling distributed tasks across multiple heterogeneous nodes in a cluster. Our empirical evaluation shows significant performance improvements relative to sequential Python in both single-node and multi-node experiments, with a performance improvement of over 20,000$\times$ when using 24 nodes and 144 GPUs in the OLCF Summit supercomputer for the Space-Time Adaptive Processing (STAP) radar application.

==> target-lang.tex <==
Aiming to deliver the benefits of distributed heterogeneous hardware
platforms to code that can be found ``in the wild'' and for which
programmers need no new training, we have focused on supporting a
widely used subset of the Python~\cite{python} language rather than
introducing a new domain-specific language.  Our approach utilizes
type hints for function parameters and return values to enhance AOT
optimizations including automatic parallelization.
%
Our \system framework currently supports the following statement
types, which are familiar to all Python and C/C++ programmers:
assignment statements, return statements, sequential for and while
loops with break and continue statements, conditional if / elif / else
statements, and calls to user-defined and built-in functions.  Most
expressions conform to the standard Python syntax and semantics.

To interface to Ray distribution framework and support CuPy-based GPU
code generation, we extended the \lang backend to support Python code
generation, namely output=Python mode (Figure~\ref{fig:overall}).
This extension also offers a variety of benefits in the \lang language
itself, e.g., it relaxes the type annotation requirements in the input
source code, and supports Python data structures/types that are not
easily convertible to C++ including heterogeneous
lists/tuples/dictionaries and ambiguous types.
%
As extensions to the \lang data type, \ttt{num} and \ttt{any} are
newly added ambiguous types that cover multiple concrete data types --
i.e., \ttt{num} as the super class of all integer, floating point, and
complex data types and \ttt{any} as the super class of all data types
and hence used as default when no type hint on function parameters and
returns.  Note that, if any/num type or Python collection is inferred
in a code region (e.g., function and loop body), output=C++ is
disabled for that code region.

